MTStereo 2.0: improved accuracy of stereo depth estimation withMax-trees

Efficient yet accurate extraction of depth from stereo image pairs is required by systems with low power resources, such as robotics and embedded systems. State-of-the-art stereo matching methods based on convolutional neural networks require intensive computations on GPUs and are difficult to deploy on embedded systems. In this paper, we propose a stereo matching method, called MTStereo 2.0, for limited-resource systems that require efficient and accurate depth estimation. It is based on a Max-tree hierarchical representation of image pairs, which we use to identify matching regions along image scan-lines. The method includes a cost function that considers similarity of region contextual information based on the Max-trees and a disparity border preserving cost aggregation approach. MTStereo 2.0 improves on its predecessor MTStereo 1.0 as it a) deploys a more robust cost function, b) performs more thorough detection of incorrect matches, c) computes disparity maps with pixel-level rather than node-level precision. MTStereo provides accurate sparse and semi-dense depth estimation and does not require intensive GPU computations like methods based on CNNs. Thus it can run on embedded and robotics devices with low-power requirements. We tested the proposed approach on several benchmark data sets, namely KITTI 2015, Driving, FlyingThings3D, Middlebury 2014, Monkaa and the TrimBot2020 garden data sets, and achieved competitive accuracy and efficiency. The code is available at https://github.com/rbrandt1/MaxTreeS.

==> experimentalSetup/flyingthings.tex <==
\renewcommand{\datasetName}{Flying Things 3D}
\renewcommand{\datasetCode}{flyingthings}





\subsubsection{\datasetName}

The \datasetName~data set contains synthetic images of textured everyday objects flying along randomized 3D trajectories and ground truth disparity maps. The background of said objects is a large textured plane. The data set contains dense ground truth disparity maps.

==> experimentalSetup/middleburry.tex <==
\renewcommand{\datasetName}{Middlebury 2014}
\renewcommand{\datasetCode}{middlebury2014}





\subsubsection{\datasetName}

The \datasetName~data set contains high resolution natural stereo pairs of indoor scenes and dense ground truth disparity maps. 



==> experimentalSetup/monkaa.tex <==
\renewcommand{\datasetName}{Monkaa}
\renewcommand{\datasetCode}{monkaa}




\subsubsection{\datasetName}

The \datasetName~data set contains synthetic, relatively un-naturalistic, images of furry objects in outdoor scenes. The data set contains dense disparity maps


==> experimentalSetup/realgarden.tex <==
\renewcommand{\datasetName}{Trimbot2020 Real Garden}
\renewcommand{\datasetCode}{realgarden}




\subsubsection{\datasetName}

The \datasetName~data set contains natural images of a garden from the viewpoint of a robot driving on the ground, and dense ground truth disparity maps. 


==> experimentalSetup/synthgarden.tex <==
\renewcommand{\datasetName}{Trimbot2020 Synthetic Garden}
\renewcommand{\datasetCode}{synthgarden}



\subsubsection{\datasetName}

The \datasetName~data set contains low-resolution synthetic stereo pairs of outdoor garden scenes with dense ground truth depth maps. They were rendered from 3D synthetic models of gardens, with different illumination and weather conditions (i.e. clear, cloudy, overcast, sunset and twilight), in the context of the TrimBot2020 project~\cite{StrisciuglioTrimbot}. The (vcam\_0, vcam\_1) stereo pairs of the Trimbot2020 {training} data set were used for evaluation. 


==> results/driving.tex <==
\renewcommand{\datasetName}{Driving}
\renewcommand{\datasetCode}{driving}

\subsection{\datasetName}

In Table~\ref{tab:\datasetCode}, we report average metric values over the~\datasetName~data set achieved by the proposed sparse and semi-dense methods in comparison with those achieved by existing methods. 

\begin{table}
\centering
\caption{Results achieved on the~\datasetName~data set.}
\label{tab:\datasetCode}
\begin{tabular}{l|cccc}
\hline
\hline
\textbf{Method} & \textbf{avgerr} & \textbf{rmse} & \textbf{Time/MP} \\
\hline
og\_bi\_sp	&	8.989	&	31.875	&	4.334	\\
og\_bi\_sd	&	38.56	&	99.84	&	4.352	\\
og\_me\_sp	&	7.812	&	28.606	&	5.265	\\
og\_me\_sd	&	31.892	&	85.679	&	3.781	\\
ng\_bi\_sp	&	8.947	&	30.519	&	4.52	\\
ng\_bi\_sd	&	22.283	&	65.827	&	3.885	\\
ng\_me\_sp	&	7.951	&	29.287	&	4.843	\\
ng\_me\_sd	&	22.093	&	64.617	&	4.14	\\
\hline
\hline
\end{tabular}
\end{table}

In Figure~\ref{fig:\datasetCode}, we show example images from the~\datasetName~data set (top row),\FiguresExplanation. 

\begin{figure}
\centering
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/a.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/b.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/a.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/b.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/e.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/f.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/g.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/h.png}
	
	\caption{Example images from the~\datasetName~data set (top row), \FiguresExplanation. }
	\label{fig:\datasetCode}
\end{figure}


==> results/flyingthings.tex <==
\renewcommand{\datasetName}{Flying Things 3D}
\renewcommand{\datasetCode}{flyingthings}

\subsection{\datasetName}

In Table~\ref{tab:\datasetCode}, we report average metric values over the~\datasetName~data set achieved by the proposed sparse and semi-dense methods in comparison with those achieved by existing methods. 

\begin{table}
\centering
\caption{Results achieved on the~\datasetName~data set.}
\label{tab:\datasetCode}
\begin{tabular}{l|cccc}
\hline
\hline
\textbf{Method} & \textbf{avgerr} & \textbf{rmse} & \textbf{Time/MP} \\
\hline
og\_bi\_sp & &  &   \\
og\_bi\_sd &  &  &   \\
og\_me\_sp &  &  &   \\
og\_me\_sd &  &  &   \\
ng\_bi\_sp & &  &   \\
ng\_bi\_sd &  &  &   \\
ng\_me\_sp &  &  &   \\
ng\_me\_sd &  &  &   \\
\hline
\hline
\end{tabular}
\end{table}

In Figure~\ref{fig:\datasetCode}, we show example images from the~\datasetName~data set (top row),\FiguresExplanation. 

\begin{figure}
\centering
	    \includegraphics[height=.17\textwidth]{Figures/\datasetCode/a.png}~\includegraphics[height=.17\textwidth]{Figures/\datasetCode/b.png}\\
	    \vspace{.1cm}
	    \includegraphics[height=.17\textwidth]{Figures/\datasetCode/a.png}~\includegraphics[height=.17\textwidth]{Figures/\datasetCode/b.png}\\
	    \vspace{.1cm}
	    \includegraphics[height=.17\textwidth]{Figures/\datasetCode/e.png}~\includegraphics[height=.17\textwidth]{Figures/\datasetCode/f.png}\\
	    \vspace{.1cm}
	    \includegraphics[height=.17\textwidth]{Figures/\datasetCode/g.png}~\includegraphics[height=.17\textwidth]{Figures/\datasetCode/h.png}
	
	\caption{Example images from the~\datasetName~data set (top row), \FiguresExplanation. }
	\label{fig:\datasetCode}
\end{figure}

==> results/kitti2015.tex <==
\renewcommand{\datasetName}{Kitti 2015}
\renewcommand{\datasetCode}{kitti2015}

\subsection{\datasetName}

In Table~\ref{tab:\datasetCode}, we report average metric values over the~\datasetName~data set achieved by the proposed sparse and semi-dense methods in comparison with those achieved by existing methods. 

\begin{table}
\centering
\caption{Results achieved on the~\datasetName~data set.}
\label{tab:\datasetCode}
\begin{tabular}{l|cccc}
\hline
\hline
\textbf{Method} & \textbf{avgerr} & \textbf{rmse} & \textbf{Time/MP} \\
\hline
ng\_bi\_sp	&	96.129	&		&	4.501	\\
ng\_me\_sp	&	95.045	&		&	5.189	\\
og\_bi\_sp	&	96.24	&		&	3.636	\\
og\_me\_sp	&	95.18	&		&	4.514	\\
ng\_bi\_sd	&	78.784	&		&	3.424	\\
ng\_me\_sd	&	75.212	&		&	4.403	\\
og\_bi\_sd	&	79.25	&		&	2.854	\\
og\_me\_sd	&	75.867	&		&	3.737	\\
\hline
\hline
\end{tabular}
\end{table}

In Figure~\ref{fig:\datasetCode}, we show example images from the~\datasetName~data set (top row),\FiguresExplanation. 

\begin{figure}
\centering
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/a.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/b.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/c.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/d.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/e.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/f.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/g.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/h.png}
	
	\caption{Example images from the~\datasetName~data set (top row), \FiguresExplanation. }
	\label{fig:\datasetCode}
\end{figure}


==> results/middleburry.tex <==
\renewcommand{\datasetName}{Middlebury 2014}
\renewcommand{\datasetCode}{middlebury2014}

\subsection{\datasetName}

In Table~\ref{tab:\datasetCode}, we report average metric values over the~\datasetName~data set achieved by the proposed sparse and semi-dense methods in comparison with those achieved by existing methods. 



\begin{table}
\centering
\caption{Results achieved on the~\datasetName~data set.}
\label{tab:\datasetCode}
\begin{tabular}{l|cccc}
\hline
\hline
\textbf{Method} & \textbf{avgerr} & \textbf{bad 2.0} & \textbf{Time/MP} & \textbf{RasPiTime/MP} \\
\hline
ng\_bi\_sp	&	14.165	&	37.397	&	2.753	&	14.752	\\
ng\_me\_sp	&	4.497	&	0.827	&	3.917	&	17.794	\\
og\_bi\_sp	&	13.012	&	36.768	&	2.279	&	14.462	\\
og\_me\_sp	&	4.005	&	1.122	&	3.365	&	17.4	\\
ng\_bi\_sd	&	15.02	&	37.241	&	2.249	&	9.221	\\
ng\_me\_sd	&	4.652	&	0.783	&	3.15	&	11.073	\\
og\_bi\_sd	&	14.093	&	36.113	&	1.787	&	8.836	\\
og\_me\_sd	&	3.621	&	1.036	&	2.549	&	10.537	\\
r200high~\cite{keselman2017intel} \\
MotionStereo~\cite{valentin2018depth} \\
ELAS\_ROB~\cite{geiger2010efficient}\\
Glstereo~\cite{Glstereo} \\
SGBM2~\cite{Hirschmuller2008}\\
SED~\cite{pena2016disparity}\\
SNCC~\cite{einecke2010two} \\
Glstereo~\cite{Glstereo} \\
LS-ELAS~\cite{jellal2017ls}\\
\hline
\hline
\end{tabular}
\end{table}

In Figure~\ref{fig:\datasetCode}, we show example images from the~\datasetName~data set (top row),\FiguresExplanation. 


\begin{figure}
\centering
	    \includegraphics[height=.17\textwidth]{Figures/\datasetCode/a.png}~\includegraphics[height=.17\textwidth]{Figures/\datasetCode/b.png}\\
	    \vspace{.1cm}
	    \includegraphics[height=.17\textwidth]{Figures/\datasetCode/c.png}~\includegraphics[height=.17\textwidth]{Figures/\datasetCode/d.png}\\
	    \vspace{.1cm}
	    \includegraphics[height=.17\textwidth]{Figures/\datasetCode/e.png}~\includegraphics[height=.17\textwidth]{Figures/\datasetCode/f.png}\\
	    \vspace{.1cm}
	    \includegraphics[height=.17\textwidth]{Figures/\datasetCode/g.png}~\includegraphics[height=.17\textwidth]{Figures/\datasetCode/h.png}
	
	\caption{Example images from the~\datasetName~data set (top row), \FiguresExplanation. }
	\label{fig:\datasetCode}
\end{figure}


==> results/monkaa.tex <==
\renewcommand{\datasetName}{Monkaa}
\renewcommand{\datasetCode}{monkaa}

\subsection{\datasetName}

In Table~\ref{tab:\datasetCode}, we report average metric values over the~\datasetName~data set achieved by the proposed sparse and semi-dense methods in comparison with those achieved by existing methods. 

\begin{table}
\centering
\caption{Results achieved on the~\datasetName~data set.}
\label{tab:\datasetCode}
\begin{tabular}{l|cccc}
\hline
\hline
\textbf{Method} & \textbf{avgerr} & \textbf{rmse} & \textbf{Time/MP} \\
\hline
og\_bi\_sp	&	4.846	&	13.389	&	1.583	\\
og\_bi\_sd	&	9.079	&	21.35	&	1.071	\\
og\_me\_sp	&	4.771	&	13.535	&	2.082	\\
og\_me\_sd	&	10.003	&	24.055	&	1.38	\\
ng\_bi\_sp	&	4.761	&	13.035	&	1.754	\\
ng\_bi\_sd	&	8.613	&	19.929	&	1.306	\\
ng\_me\_sp	&	4.669	&	12.935	&	3.782	\\
ng\_me\_sd	&	9.053	&	21.255	&	4.279	\\
\hline
\hline
\end{tabular}
\end{table}

In Figure~\ref{fig:\datasetCode}, we show example images from the~\datasetName~data set (top row),\FiguresExplanation. 

\begin{figure}
\centering
	    \includegraphics[height=.13\textwidth]{Figures/\datasetCode/a.png}~\includegraphics[height=.13\textwidth]{Figures/\datasetCode/b.png}\\
	    \vspace{.1cm}
	    \includegraphics[height=.17\textwidth]{Figures/\datasetCode/c.png}~\includegraphics[height=.17\textwidth]{Figures/\datasetCode/d.png}\\
	    \vspace{.1cm}
	    \includegraphics[height=.13\textwidth]{Figures/\datasetCode/e.png}~\includegraphics[height=.13\textwidth]{Figures/\datasetCode/f.png}\\
	    \vspace{.1cm}
	    \includegraphics[height=.13\textwidth]{Figures/\datasetCode/g.png}~\includegraphics[height=.13\textwidth]{Figures/\datasetCode/h.png}
	
	\caption{Example images from the~\datasetName~data set (top row), \FiguresExplanation. }
	\label{fig:\datasetCode}
\end{figure}


==> results/realgarden.tex <==
\renewcommand{\datasetName}{Trimbot2020 Real Garden}
\renewcommand{\datasetCode}{realgarden}

\subsection{\datasetName}

In Table~\ref{tab:\datasetCode}, we report average metric values over the~\datasetName~data set achieved by the proposed sparse and semi-dense methods in comparison with those achieved by existing methods. 


\begin{table}
\centering
\caption{Results achieved on the~\datasetName~data set.}
\label{tab:\datasetCode}
\begin{tabular}{l|cccc}
\hline
\hline
\textbf{Method} & \textbf{avgerr} & \textbf{rmse} & \textbf{Time/MP} \\
\hline
ng\_bi\_sd	&	3.166	&	22.564	&	3.805	\\
ng\_bi\_sp	&	2.84	&	21.976	&	5.272	\\
ng\_me\_sd	&	3.052	&	23.394	&	3.54	\\
ng\_me\_sp	&	2.968	&	23.14	&	4.874	\\
og\_bi\_sd	&	2.999	&	22.848	&	3.012	\\
og\_bi\_sp	&	2.916	&	22.659	&	4.167	\\
og\_me\_sd	&	2.988	&	23.034	&	2.653	\\
og\_me\_sp	&	2.949	&	22.929	&	3.702	\\
\hline
\hline
\end{tabular}
\end{table}




In Figure~\ref{fig:\datasetCode}, we show example images from the~\datasetName~data set (top row),\FiguresExplanation. 

\begin{figure}
\centering
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/a.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/b.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/c.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/d.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/e.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/f.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/g.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/h.png}
	
	\caption{Example images from the~\datasetName~data set (top row), \FiguresExplanation. }
	\label{fig:\datasetCode}
\end{figure}


==> results/synthgarden.tex <==
\renewcommand{\datasetName}{Trimbot2020 Synthetic Garden}
\renewcommand{\datasetCode}{synthgarden}

\subsection{\datasetName}

In Table~\ref{tab:\datasetCode}, we report average metric values over the~\datasetName~data set achieved by the proposed sparse and semi-dense methods in comparison with those achieved by existing methods. 

\begin{table}
\centering
\caption{Results achieved on the~\datasetName~data set.}
\label{tab:\datasetCode}
\begin{tabular}{l|cccc}
\hline
\hline
\textbf{Method} & \textbf{avgerr} & \textbf{rmse} & \textbf{Time/MP} \\
\hline
og\_bi\_sp	&	6.068	&	9.698	&	2.719	\\
og\_bi\_sd	&	5.271	&	8.957	&	2.207	\\
og\_me\_sp	&	6.003	&	9.637	&	2.892	\\
og\_me\_sd	&	5.2	&	8.881	&	1.827	\\
ng\_bi\_sp	&	6.053	&	9.688	&	2.757	\\
ng\_bi\_sd	&	5.225	&	8.907	&	1.841	\\
ng\_me\_sp	&	5.993	&	9.63	&	2.959	\\
ng\_me\_sd	&	5.152	&	8.826	&	1.9	\\
\hline
\hline
\end{tabular}
\end{table}

In Figure~\ref{fig:\datasetCode}, we show example images from the~\datasetName~data set (top row),\FiguresExplanation. 

\begin{figure}
\centering
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/a.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/b.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/c.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/d.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/e.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/f.png}\\
	    \vspace{.1cm}
	    \includegraphics[width=.24\textwidth]{Figures/\datasetCode/g.png}~\includegraphics[width=.24\textwidth]{Figures/\datasetCode/h.png}
	
	\caption{Example images from the~\datasetName~data set (top row), \FiguresExplanation. }
	\label{fig:\datasetCode}
\end{figure}



\begin{table*}[t]
  \centering
  \begin{tabular}{rcccccccccccccccccccccccccccc}
    \toprule
     & \multicolumn{2}{c}{Middleburry} & \multicolumn{2}{c}{Kitti2015} 
      & \multicolumn{2}{c}{Real Garden} & \multicolumn{2}{c}{Synth Garden} 
       & \multicolumn{2}{c}{Driving} & \multicolumn{2}{c}{Monkaa}
       & \multicolumn{2}{c}{Flying Things} \\
     
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15}
    
     & \multicolumn{1}{c}{avgerr} & \multicolumn{1}{c}{bad 2.0} 
     & \multicolumn{1}{c}{avgerr} & \multicolumn{1}{c}{bad 2.0} 
      & \multicolumn{1}{c}{avgerr} & \multicolumn{1}{c}{bad 2.0} 
       & \multicolumn{1}{c}{avgerr} & \multicolumn{1}{c}{bad 2.0} 
        & \multicolumn{1}{c}{avgerr} & \multicolumn{1}{c}{rmse} 
         & \multicolumn{1}{c}{avgerr} & \multicolumn{1}{c}{rmse} 
          & \multicolumn{1}{c}{avgerr} & \multicolumn{1}{c}{rmse} \\
     
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11} \cmidrule(lr){12-12} \cmidrule(lr){13-12} \cmidrule(lr){14-14} \cmidrule(lr){15-15} \\																												
																													
og\_bi\_sp	&	14.165	&	37.397	&	96.129	&		&	3.166	&	22.564	&	6.068	&	9.698	&	8.989	&	31.875	&	4.846	&	13.389	&		&		\\
og\_bi\_sd	&	4.497	&	0.827	&	95.045	&		&	2.84	&	21.976	&	5.271	&	8.957	&	38.56	&	99.84	&	9.079	&	21.35	&		&		\\
og\_me\_sp	&	13.012	&	36.768	&	96.24	&		&	3.052	&	23.394	&	6.003	&	9.637	&	7.812	&	28.606	&	4.771	&	13.535	&		&		\\
og\_me\_sd	&	4.005	&	1.122	&	95.18	&		&	2.968	&	23.14	&	5.2	&	8.881	&	31.892	&	85.679	&	10.003	&	24.055	&		&		\\
ng\_bi\_sp	&	15.02	&	37.241	&	78.784	&		&	2.999	&	22.848	&	6.053	&	9.688	&	8.947	&	30.519	&	4.761	&	13.035	&		&		\\
ng\_bi\_sd	&	4.652	&	0.783	&	75.212	&		&	2.916	&	22.659	&	5.225	&	8.907	&	22.283	&	65.827	&	8.613	&	19.929	&		&		\\
ng\_me\_sp	&	14.093	&	36.113	&	79.25	&		&	2.988	&	23.034	&	5.993	&	9.63	&	7.951	&	29.287	&	4.669	&	12.935	&		&		\\
ng\_me\_sd	&	3.621	&	1.036	&	75.867	&		&	2.949	&	22.929	&	5.152	&	8.826	&	22.093	&	64.617	&	9.053	&	21.255	&		&		\\
																													
     \bottomrule
  \end{tabular}
\end{table*}




==> tableAccuracyOld.tex <==

\begin{table*}[!t]
  \centering
\renewcommand{\arraystretch}{1.3}  
 \setlength{\tabcolsep}{3pt}
  \caption{Results expressed in \textit{avgerr}, except Kitty2015 Test which are expressed in \textit{D-all-est}. Average prediction density is reported in brackets. Entries without density specification are 100\% dense. Entries with ?\% density specification have unknown density. We mark with $^*$ the results that were (possibly) computed on a different set of images than we used for evaluation. We mark with $^+$ that result was taken from respective benchmark website. We mark with $^T$ results that were (possibly) computed using a different metric computation approach.}
  \label{tab:accuracyResults}
\setlength{\tabcolsep}{2pt}
\tinysize
  \begin{tabular}{rccccccccc}
 
    \toprule
     &\multicolumn{2}{c}{\textbf{Middlebury}} &\multicolumn{2}{c}{\textbf{Kitti2015}} 
      &\multicolumn{1}{c}{\textbf{Real Garden}} &\multicolumn{1}{c}{\textbf{Synth Garden}} 
       &\multicolumn{1}{c}{\textbf{Driving}} &\multicolumn{1}{c}{\textbf{Monkaa}}
       &\multicolumn{1}{c}{\textbf{Flying Things}} \\
       
     &\multicolumn{1}{c}{Train} &\multicolumn{1}{c}{Test}  &\multicolumn{1}{c}{Train} &\multicolumn{1}{c}{Test} &\multicolumn{1}{c}{}  
     &\multicolumn{1}{c}{}  
     &\multicolumn{1}{c}{} 
     &\multicolumn{1}{c}{} 
     &\multicolumn{1}{c}{} \\
     
    \cmidrule(lr){2-3}     \cmidrule(lr){4-5}           \cmidrule(lr){6-6}     \cmidrule(lr){7-7}     \cmidrule(lr){8-8} 		
    \cmidrule(lr){9-9}     \cmidrule(lr){10-10} 

\textbf{MTS2.0 (sparse)}&\textbf{2.35}$^+$(3\%)&\textbf{9.36}$^+$(3\%)& 1.35(4\%) &7.83$^+$(4\%)&3.08(5\%)&5.22(6\%)&\textbf{5.36}(3\%)&\textbf{3.83}(4\%)&\textbf{1.7}(6\%)\\
\textbf{MTS2.0 (semi-dense)}&6.51(24\%)&\---&$2.24$(25\%)&\---&3.72(20\%)&7.04(19\%)&7.38(15\%)&6.54(25\%)&2.61(30\%) \\
MTS1.0 (sparse)&5.47$^+$(2\%) &15.5$^+$(2\%)&1.58(2\%)&8.92$^+$(3\%)&2.48(2\%)&7.32(2\%)& 8.8(1\%)&7.22(3\%)&3.03(4\%)\\
MTS1.0 (semi-dense)&17.47(57\%) &\---&4.47(44\%)&\---& 3.78(18\%)&12.8(14\%)&16.2(38\%)&15.41(40\%)&6.93(58\%)\\
SGBM1 \cite{Hirschmuller2008}&7.83$^+$(67\%)&16.3$^+$(63\%)&1.45(84\%)&\---&2.61(89\%)&4.77(92\%)&16.06(70\%)&11.37(81\%)&5.14(86\%)\\
SGBM2 \cite{Hirschmuller2008}&8.92$^{+*}$(83\%)&15.9$^{+*}$(77\%)&\textbf{1.27}(82\%)&\textbf{5.86}$^+$(90\%)&2.16(90\%)&\textbf{4.67}(90\%)&15.72(64\%)&10.5(78\%)&4.58(85\%)\\
ELAS\_ROB \cite{geiger2010efficient} &10.5$^{+*}$&13.4$^{+*}$&1.49(99\%)&9.67$^+$&\textbf{2.06}&7.02&11.71&17.75&7.46\\
FPGA Stereo \cite{honegger2017embedded}&\---&\---&\---&\---&2.94\cite{pu2019sdf}&11.41\cite{pu2019sdf}&\---&\---&\---\\
 \hline 
DispNet \cite{mayer2016large}&\---&\---&\textbf{0.68}\cite{mayer2016large}&4.34$^+$&\textbf{1.35}\cite{pu2019sdf}&\textbf{6.28}\cite{pu2019sdf}&\textbf{15.62}$^*$\cite{mayer2016large}&\textbf{5.78}\cite{mayer2016large}&1.68\cite{mayer2016large} \\
EdgeStereo \cite{song2019edgestereo}&\textbf{2.00}$^+$&\textbf{3.72}$^+$&2.07(?\%)\cite{song2019edgestereo}&\textbf{2.08}$^+$&\--- &\---&\---&\---&\textbf{0.74}$^{*T}$(?\%)\cite{song2019edgestereo}\\
iResNet \cite{liang2017learning}&\---&\---&1.21(?\%)\cite{song2019edgestereo}&2.44$^T$(?\%)\cite{song2019edgestereo}&\---&\---&\---&\---&0.95$^{*T}$(?\%)\cite{song2019edgestereo}\\
     \bottomrule
  \end{tabular}
\end{table*}




\begin{table*}[!h]
  \centering
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.3}  
   \caption{Results on the Middlebury training benchmark expressed in \textit{avgerr}. Results of MTStereo 2.0 are bold. All results taken from respective benchmark website, except that of Semi-Dense. We mark with $^*$ the results that were computed on a different set of images than we used for evaluation.}
  \label{tab:accuracyResultsMiddlebury}
   \begin{tabular}{ccccccccccccc}
    \toprule
   R-NCC \cite{li2019removal}&DAWA-F &MotionStereo\cite{valentin2018depth} &INTS \cite{huang2016image}&SGM \cite{hirschmuller2007stereo} &\textbf{Sparse} &MPSV \cite{bricola2016morphological}&SNCC \cite{einecke2010two} & \textbf{Semi-Dense}\\

 \cmidrule(lr){1-1}  \cmidrule(lr){2-2}     \cmidrule(lr){3-3}     \cmidrule(lr){4-4}     \cmidrule(lr){5-5}     \cmidrule(lr){6-6}     \cmidrule(lr){7-7}     \cmidrule(lr){8-8} 	 \cmidrule(lr){9-9}  \cmidrule(lr){10-10} %	 \cmidrule(lr){10-10} 	 \cmidrule(lr){11-11} 	 \cmidrule(lr){12-12} 	
 0.59(34\%) &1.56$^*$(62\%) &1.72$^*$(46\%) &1.99$^*$(76\%)&2.06(58\%) &2.35(3\%) &2.83$^*$(39\%)&3.25$^*$(62\%) & 6.51(24\%)\\
     \bottomrule
  \end{tabular}
\end{table*}





\begin{table*}[!h]
  \centering
  \renewcommand{\arraystretch}{1.3}  
   \caption{Results on the Middlebury test benchmark expressed in \textit{avgerr}. Results of MTStereo 2.0 are bold. All results taken from respective benchmark website. We mark with $^*$ the results that were computed on a different set of images than we used for evaluation.}
  \label{tab:accuracyResultsMiddleburyTest}
   \begin{tabular}{ccccccccccc}
    \toprule
    R-NCC \cite{li2019removal}&DAWA-F &SGM \cite{hirschmuller2007stereo}&INTS \cite{huang2016image}&MPSV \cite{bricola2016morphological}&MotionStereo\cite{valentin2018depth}  &SNCC \cite{einecke2010two} &\textbf{Sparse}\\

 \cmidrule(lr){1-1}  \cmidrule(lr){2-2}     \cmidrule(lr){3-3}     \cmidrule(lr){4-4}     \cmidrule(lr){5-5}     \cmidrule(lr){6-6}     \cmidrule(lr){7-7}     \cmidrule(lr){8-8} \cmidrule(lr){9-9} 	  %	 \cmidrule(lr){10-10} 	 \cmidrule(lr){11-11} 	 \cmidrule(lr){12-12} 	
0.93(28\%)&2.29$^*$(53\%)& 2.50(50\%) & 2.87$^*$(74\%) & 3.21$^*$(31\%) & 3.30$^*$(38\%) & 3.96$^*$(55\%) & 9.36(3\%)\\
 
     \bottomrule
  \end{tabular}
\end{table*}
